Learning Activation Functions for Sparse Neural Networks

Sparse Neural Networks (SNNs) can potentially demonstrate similar performance to their dense counterparts while saving significant energy and memory at inference. However, the accuracy drop incurred by SNNs, especially at high pruning ratios, can be an issue in critical deployment conditions. While recent works mitigate this issue through sophisticated pruning techniques, we shift our focus to an overlooked factor: hyperparameters and activation functions. Our analyses have shown that the accuracy drop can additionally be attributed to (i) Using ReLU as the default choice for activation functions unanimously, and (ii) Fine-tuning SNNs with the same hyperparameters as dense counterparts. Thus, we focus on learning a novel way to tune activation functions for sparse networks and combining these with a separate hyperparameter optimization (HPO) regime for sparse networks. By conducting experiments on popular DNN models (LeNet-5, VGG-16, ResNet-18, and EfficientNet-B0) trained on MNIST, CIFAR-10, and ImageNet-16 datasets, we show that the novel combination of these two approaches, dubbed Sparse Activation Function Search, short: SAFS, results in up to 15.53%, 8.88%, and 6.33% absolute improvement in the accuracy for LeNet-5, VGG-16, and ResNet-18 over the default training protocols, especially at high pruning ratios. Our code can be found at https://github.com/automl/SAFS

==> Misc.tex <==
\begin{table*}[hbpt]
  \centering
  \caption{Datasets and models used in experiments.} 
  \label{tab:Experimental_Setup:ArchitectureConfig}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{cc|ccc|c}
    \hline
     \multicolumn{2}{c|}{\textbf{Dataset}}  & \multicolumn{3}{c|}{CIFAR-10} & ImageNet 32$\times$32\\ \hline
     
    \multicolumn{2}{c|}{\textbf{Network}}  & VGG-16 & ResNet-18 & EfficientNet & LocalViT\\ \hline
                & Epoch (\#) & 200 & 200 & 350 & \\
         & Learning Rate (\textit{lr}) & 0.1 &  0.1 & 0.256 & \\
\textbf{Default} & \multirow{2}{*}{\textit{lr} Scheduler} & Step: 'size': 70 & Step: 'size': 70 & Decays by 0.97 & \\
 \textbf{Training} &  &  'gamma': 0.&  'gamma': 0.1 & every 2.4 epochs & \\
 \textbf{Configuration} & Weight Decay & 5e-4&  5e-4 & 1e-5 & \\ 
 & Momentum & 0.9 & 0.9 & 0.9 & \\ 
                & Optimizer & SGD & SGD & RMSProp & \\ \hline
                & Train Time (GPU Hours) & 1.8 & 4.0 & & \\ \hline
\end{tabular}}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[htbp]
\centering
\resizebox{\columnwidth}{!}{   
\begin{tikzpicture} [spy using outlines= {circle, magnification=2, connect spies}]
    \begin{axis}[ 
        ymin=87,
        ymax=94,
        xmin=89,
        xmax=100,
        width=\columnwidth,
        height=0.75\columnwidth,
        ylabel={Test Accuracy (\%)},
        xlabel={Pruning Ratio (\%)},
        ylabel near ticks,
        xlabel near ticks,
        grid=major, 
        xtick={90,95,99},
        xticklabels = {90,95,99},
        grid style={dashed,gray!60},
        legend style={draw=black,at={(1.31,0.525)}, text opacity = 1,row sep=-1pt, font=\fontsize{9}{6}\selectfont},
        x tick label style={rotate=0,anchor=north}
        ]
        \addplot [smooth,mark=square*, mark size=2pt, red, very thick, draw=red] coordinates {(90,92.65) (95,92.65) (99,87.61)};
        \addplot [smooth, mark=diamond*, mark size=3pt, teal, thick, draw=teal] coordinates {(90,92.44)(99,88.42)};
        \addplot [smooth, mark=*, mark size=3pt, olive, thick, draw=olive] coordinates {(90,92.45)(99,88.28)};
        \addplot [smooth,mark=x, mark size=4pt, black, very thick, draw=black] coordinates {(90,93.19) (99,88.26)};
        \addplot [smooth, mark=pentagon*, mark size=4pt, cyan, very thick, draw=black] coordinates {(90,91.875) (95,88.99) (99,80.72)};
        \addplot [smooth,mark=triangle*, mark size=4pt, violet, very thick, draw=violet] coordinates {(90,92.875) (95,90.99) (99,82.72)};
    \legend{ReLU, PReLU, Swish, PSwish, SeLU, SRS}    
    \end{axis}
    \end{tikzpicture}
}
\caption{CIFAR-10 test accuracy on sparse VGG-16 with different \afs.} 
\label{fig:motivation:AF}
\end{figure}


%%%%%%%%%%%%%%%%%


\section{Results of Gradient Flow}
\label{Appendix:Gradient_Flow}

\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cccc}
%\includegraphics[width=\columnwidth]{Figures/GF/1.eps} & 
%\includegraphics[width=\columnwidth]{Figures/GF/2.eps}& 
%\includegraphics[width=\columnwidth]{Figures/GF/3.eps}& 
%\includegraphics[width=\columnwidth]{Figures/GF/4.eps}
\\
 \textbf{Conv. Layer \#1}& \textbf{Conv. Layer \#2}& \textbf{Conv. Layer \#3} &\textbf{Conv. Layer \#4}
\\
%\includegraphics[width=\columnwidth]{Figures/GF/5.eps}& 
%\includegraphics[width=\columnwidth]{Figures/GF/6.eps}& 
%\includegraphics[width=\columnwidth]{Figures/GF/7.eps}& 
%\includegraphics[width=\columnwidth]{Figures/GF/8.eps}
\\
 \textbf{Conv. Layer \#5}& \textbf{Conv. Layer \#6}& \textbf{Conv. Layer \#7} &\textbf{Conv. Layer \#8}
\\
%\includegraphics[width=\columnwidth]{Figures/GF/8.eps}& 
%\includegraphics[width=\columnwidth]{Figures/GF/10.eps}& 
%\includegraphics[width=\columnwidth]{Figures/GF/11.eps}& 
%\includegraphics[width=\columnwidth]{Figures/GF/12.eps}
\\
 \textbf{Conv. Layer \#9}& \textbf{Conv. Layer \#10}& \textbf{Conv. Layer \#11} &\textbf{Conv. Layer \#12}
\\
& 
%\multicolumn{2}{c}{\includegraphics[width=\columnwidth]{Figures/GF/13.eps}}
& 
\\
 %& \multicolumn{2}{c}{\textbf{Conv. Layer \#13}}& 
\\
\end{tabular}
}
\captionof{figure}{Illustrating the gradient flow of training VGG-16 on CIFAR-10 with different activation functions. The pruning ratio is 99\%.} 
\label{fig:Appendix:GF}
\end{table}


%%%%%%%%%%%%%

\begin{figure}[htbp]
\centering
\resizebox{\columnwidth}{!}{
\begin{tikzpicture}[spy using outlines=
	{circle, magnification=2, connect spies}]
    \begin{axis}[
        height= 0.75\columnwidth,
        width= \columnwidth,
        xmin=1, xmax=200,
        ymin=10, ymax=83,
        xlabel= \textbf{Epoch (\#)},
        ylabel= \textbf{Test Accuracy (\%)},
        enlarge y limits=true,   
        ylabel shift = -3 pt,
        ymajorgrids=true,
        xmajorgrids=true,
        grid style=dashed,
        ytick = {40,50,60,70,80,90},     
        legend style={at={(0.5,-0.2)},anchor=north, nodes={scale=0.75,transform shape}}, 
        legend pos=south east,
        label style={font=\small}, tick label style={font=\small} 
        ]
    \addplot[blue, smooth, very  thick] table[x=Epoch,y=without_HPO,col sep=comma] {Figures/AF_Train_HPO_Motivation.csv};
    \addplot[red, smooth, very  thick] table[x=Epoch,y=HPO,col sep=comma] {Figures/AF_Train_HPO_Motivation.csv};
    %\addplot[teal, smooth, dashed, very thick] table[x=Epoch,y=VGG-Dense,col sep=comma] {Figures/AF_Train_HPO_Motivation.csv};
\legend{Fine-tuning with dense hyperparameters, Fine-tuning with optimized hyperparameters}

\node[] at (axis cs: 120,50) {\scriptsize \textbf{$2.85\%$}};
\addplot [<->, black, thick] coordinates {(134,46)  (134,53)}; 

\coordinate (spypoint) at (axis cs:160,80);
\coordinate (magnifyglass) at (axis cs:160,50);

\spy [olive, size=1.5cm] on (spypoint)
   in node[fill=white] at (magnifyglass);
   
\end{axis}
\end{tikzpicture}
}

\caption{Fine-tuning sparse VGG-16 on CIFAR-10 with different training hyperparameters. The pruning ratio is 99\%.} 
\label{fig:motivation:HPO}
\end{figure}


%%%%%%%%%%%%

\begin{table}[hbpt]
\centering
\caption{Evaluating the effectiveness of \ourname at various pruning ratios.}
\label{tab:Sensitivity_pruning_ratio}
\resizebox{0.4\linewidth}{!}{%
\begin{tabular}{cccc}
\hline
\multirow{2}{*}{\textbf{CNN Architecture}} & \multicolumn{3}{c}{\textbf{Pruning Ratio}}\\ \cline{2-4}

& 90\% & 95\%& 99\% \\ \hline

VGG-16 with ReLU  & \multirow{ 2}{*}{79.33\%} & \multirow{ 2}{*}{72.51\%} & \multirow{ 2}{*}{70.32\%}  \\ 
(baseline) &  &  &   \\ \cline{1-1}
VGG-16 + \ourname & 80.98\% \textbf{\color{blue}(+1.65\%)} & 79.46\% \textbf{\color{blue}(+7.45\%)}  &  79.2\% \textbf{\color{blue}(+8.88\%)}  \\
\hline
\end{tabular}}
\end{table}

%%%%%%%%%%%%%
\begin{table*}[htbp]
\centering
\captionsetup{justification=centering}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{cc}

\includegraphics[width=0.48\textwidth]{Figures/Insight_VGG.pdf}&
\includegraphics[width=0.47\textwidth]{Figures/Insight_ResNet.pdf}
\\
\textbf{(a)  VGG-16} & \textbf{(b) ResNet-18} 
\\

\end{tabular}}
\captionof{figure}{Frequency of Occurring unary operator in the first learning stage ($\alpha=\beta=1$) for (a) VGG-16 and (b) ResNet-18 trained on CIFAR-10.}
  \label{fig:Insights}
\end{table*}

%%%%%%%%%
\begin{figure}[hbpt]
\centering

      \begin{tikzpicture}[scale=0.5]
      \begin{axis}[
        ymin=0, ymax=10,
        xmin=0,xmax=110,
        grid=major, 
        grid style={dashed, gray!60},
        xlabel=\small	\textbf{Compression Ratio ($\times$) }, 
        ylabel=\small	 \textbf{Accuracy Improvement (\%)},
        ylabel near ticks,
        xlabel near ticks,
        legend style={at={(0.5,0.0)},anchor=north},
        legend style={draw=black, at={(1.51,1.)}, text opacity = 1,row sep=0.8pt, font=\fontsize{7.5}{6}\selectfont},
         x tick label style={rotate=0,anchor=north},
        ]
        
        \addplot [mark=square*, mark size=4pt, red, thick, draw=black ] coordinates {(100,8.88) (20,7.45) (10,1.65)};

        \addplot [mark=diamond*, only marks, mark size=5pt, cyan, thick,draw=black] coordinates {(13.88,3)};

        \addplot [mark=square*, mark size=4pt, blue, thick, draw=black ] coordinates {(20,2.2)};

        \addplot [mark=oplus*, only marks, mark size=5pt, green, thick,draw=black] coordinates {(100,6.33)};

        \addplot [mark=x, mark size=5pt, only marks, gray, line width=2pt,draw=black] coordinates {(100,3.91)};

        \addplot [fill, mark=pentagon*, only marks, mark size=5pt, teal, thick,draw=black] coordinates {(7.14,1)};

        \addplot [fill, mark=halfcircle*, only marks, mark size=5pt, orange,draw=black] coordinates {(45.73,2.64)}; 

        \addplot [fill, mark= halfsquare left*, only marks, mark size=6pt, yellow,draw=black] coordinates {(16, 0.3)};

        \addplot [mark=triangle*, only marks, mark size=6pt, brown, thick,draw=black] coordinates {(20,4.4)};
       
        \legend{VGG-16+\texttt{SAFS} (Ours), VGG-16+\citep{huang-wacv18}, VGG-16+Hydra \citep{sehwag-neurips20}, ResNet-18+\texttt{SAFS} (Ours), ResNet-18+Hydra \citep{sehwag-neurips20}, ResNet-18+One-Shot \citep{hubens-icip22}, ResNet-18+TAS \citep{loni-date22}, ResNet-18+TRQ \citep{li-aaai22}, DeepMaker \citep{loni-micro20} }
      \end{axis}
    \end{tikzpicture}
\caption{Showing the accuracy improvement (\%) vs. the number of network parameters (\#Params) trained on CIFAR-10 for various sparse and quantized  architectures.} 
\label{Fig:Experiments:Hardware}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Transferability of Results}
\label{Appendix:Transfer_to_ImageNet}

\cref{tab:Transfer_to_ImageNet}


\begin{table}[htbp]
\centering
\caption{Transferability of \ourname's results on ImageNet-16 to the original ImageNet-1k dataset. }
\label{tab:Transfer_to_ImageNet}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c}
\hline
\textbf{ImageNet-16 Dataset} &  \textbf{Accuracy (Top-1 / Top-5)} \\ \hline
Dense Model  (EfficientNet-B0$^\ddagger$) &  76.3\% / 93.1\% \\
Pruning without Fine-tuning &  0.1\% / 0.5\% \\
Vanilla Pruning (\underline{Baseline}) &  25\% on epoch 5 / .\%\\
\ourname (Ours) &  12\% on epoch 12 \textbf{\color{blue}(+.\%)} / .\% \textbf{\color{blue}(+.\%)} \\ \hline
\multicolumn{2}{l}{$^\ddagger$ The model and original hyper-parameters are based on \url{https://github.com/lukemelas/EfficientNet-PyTorch}.} \\ \hline
\end{tabular}%
}
\end{table}

==> content/Reproducibility_Checklist.tex <==
\section{Reproducibility Checklist}
\label{Sec:Reproducibility_Checklist}

\begin{enumerate}
%
\item For all authors\dots
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    %
    \answerYes{}
    %
  \item Did you describe the limitations of your work?
    %
    \answerYes{}
    %
  \item Did you discuss any potential negative societal impacts of your work?
    %
    \answerYes{}
    %
  \item Have you read the ethics author's and review guidelines and ensured that your paper conforms to them? \url{https://automl.cc/ethics-accessibility/}
    %
    \answerYes{}
    %
  \end{enumerate}
  %
\item If you are including theoretical results\dots
  %
  \begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    %
    \answerNA{}
    %
  \item Did you include complete proofs of all theoretical results?
    %
    \answerNA{}
    %
  \end{enumerate}
  %
\item If you ran experiments\dots
  %
  \begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results, including all requirements (e.g., \texttt{requirements.txt} with explicit version), an instructive \texttt{README} with installation, and execution commands (either in the supplemental material or as a \textsc{url})?
    %
    \answerYes{}
    %
  \item Did you include the raw results of running the given instructions on the given code and data?
    %
    \answerYes{}
    %
  \item Did you include scripts and commands that can be used to generate the figures and tables in your paper based on the raw results of the code, data, and instructions given?
    %
    \answerYes{}
    %
  \item Did you ensure sufficient code quality such that your code can be safely executed and the code is properly documented?
    %
    \answerYes{}
    %
  \item Did you specify all the training details (e.g., data splits, pre-processing, search spaces, fixed hyperparameter settings, and how they were chosen)?
    %
    \answerYes{}
    %
  \item Did you ensure that you compared different methods (including your own) exactly on the same benchmarks, including the same datasets, search space, code for training and hyperparameters for that code?
    %
    \answerYes{\cref{appendix:search-algorithms} compares different search methods for solving \cref{eq:Method:Objective_1}. }
    %
  \item Did you run ablation studies to assess the impact of different components of your approach?
    %
    \answerYes{\cref{tab:Ablation:AF_HPO}}
    %
  \item Did you use the same evaluation protocol for the methods being compared?
    %
    \answerYes{}
    %
  \item Did you compare performance over time?
    %
    \answerNA{}
    %
  \item Did you perform multiple runs of your experiments and report random seeds?
    %
    \answerYes{}
    %
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    %
    \answerYes{}
    %
  \item Did you use tabular or surrogate benchmarks for in-depth evaluations?
    %
    \answerNo{}
    %
  \item Did you include the total amount of computing and the type of resources used (e.g., type of \textsc{gpu}s, internal cluster, or cloud provider)?
    %
    \answerYes{\cref{Sec:Experimental_Setup:tab:HW_Spec} lists the type of resources used in this paper. \cref{Appendix:Reproducibility} reports the amount of compute time for the activation function optimization.}
    %
  \item Did you report how you tuned hyperparameters, and what time and
    resources this required (if they were not automatically tuned by your AutoML method, e.g. in a \textsc{nas} approach; and also hyperparameters of your
    own method)?
    %
    \answerYes{}
    %
  \end{enumerate}
  %
\item If you are using existing assets (e.g., code, data, models) or
  curating/releasing new assets\dots
  %
  \begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    %
    \answerYes{}
    %
  \item Did you mention the license of the assets?
    %
    \answerYes{}
    %
  \item Did you include any new assets either in the supplemental material or as
    a \textsc{url}?
    %
    \answerNA{}
    %
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    %
    \answerNA{}
    %
  \item Did you discuss whether the data you are using/curating contains
    personally identifiable information or offensive content?
    %
    \answerNA{}
    %
  \end{enumerate}
  %
\item If you used crowdsourcing or conducted research with human subjects\dots
  %
  \begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    %
    \answerNA{}
    %
  \item Did you describe any potential participant risks, with links to
    Institutional Review Board (\textsc{irb}) approvals, if applicable?
    %
    \answerNA{}
    %
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    %
    \answerNA{}
    %
  \end{enumerate}
\end{enumerate}



